Abstraction Engineering

Modern software-based systems operate under rapidly changing conditions and face ever-increasing uncertainty. In response, systems are increasingly adaptive and reliant on artificial-intelligence methods. In addition to the ubiquity of software with respect to users and application areas (e.g., transportation, smart grids, medicine, etc.), these high-impact software systems necessarily draw from many disciplines for foundational principles, domain expertise, and workflows. Recent progress with lowering the barrier to entry for coding has led to a broader community of developers, who are not necessarily software engineers. As such, the field of software engineering needs to adapt accordingly and offer new methods to systematically develop high-quality software systems by a broad range of experts and non-experts. This paper looks at these new challenges and proposes to address them through the lens of Abstraction. Abstraction is already used across many disciplines involved in software development -- from the time-honored classical deductive reasoning and formal modeling to the inductive reasoning employed by modern data science. The software engineering of the future requires Abstraction Engineering -- a systematic approach to abstraction across the inductive and deductive spaces. We discuss the foundations of Abstraction Engineering, identify key challenges, highlight the research questions that help address these challenges, and create a roadmap for future research.

==> _text_mine.tex <==
\section{Solution strategies}
\label{section:solution_strategies}

  The four key challenges we have identified above are tackled -- partially -- by solution strategies involving abstractions in different sub-disciplines of software and systems engineering (including, but not limited to, formal methods, model-driven engineering, machine learning and AI, or software~/ systems product-line engineering). 
  Below, we provide some illustrative examples.
  Note how these examples stem from different sub-disciplines.\draft{Need to make sure they do and indicate where each comes from\ldots}

  \begin{enumerate}
    \item \emph{Complexity.}
    
          The \emph{complexity} of AI-based systems and their environments can be partially addressed by capturing key abstractions of the system environment (e.g., roads, pavements, pedestrians\ldots) so that a broad variety of large, diverse, and realistic test scenarios can be automatically generated using evolutionary computation and model generation. 
          While this may not be able to provide the level of assurance that model-based testing can provide for more traditionally engineered systems, the level of assurance can be increased by generating as broad and diverse a range of scenarios as possible.
          \draft{Which sub-discipline(s) does this come from?}
    
          A personalized information service needs to deal with complexity of essentially unbounded knowledge in your life. In order to maintain the ergonomy of interaction it needs to arrive at \emph{personalized abstractions} that present only the required information, in a manner that is comprehensible for the individual user. Furthermore, when the user is interested in more detailed information as provided, automatic refinement of the presented abstractions is needed. Note that the activities of abstraction and refinement of information are key activities in Abstraction Engineering.       
          \draft{Which sub-discipline(s) does this come from?}
    
          \begin{itemize}
              \item Some of this is `bread and butter': we know how to build modelling languages/notations and domain-relevant abstractions that can hide complexity as well as transformations for translating these into executable software. It is worth mentioning that we can provide different notations for different profiles, all linked to the same metamodel.
              \item We also have existing and emerging technology to support collaboration between stakeholders with different views (though  reconciliation where conflict occurs and possibly across abstraction levels needs more support)\draft{Add some references here} as well as their efficient near-realtime collaboration\draft{possibly cite web-based modelling}
              \item It remains to better support the human in the loop by finding better ways of identifying the \emph{right} abstractions.
              \item Having the right abstractions and models to communicate information pertaining to trustworthiness of the DT remains an open challenge -- we know how to build abstractions, and GSN-style languages may be particularly promising here -- but we don't know the specific abstractions we need. We need ways to expose complexity/causality in a DT in limited but useful ways to explain and document decision making.
          \end{itemize}
          \draft{Which sub-discipline(s) does this come from?}
    
    \item \emph{Compositionality.}
    
          Issues of \emph{compositionality} and \emph{reuse} can be addressed by capturing key abstractions about how AI-based components are engineered and how they may interact with other components.
          This will enable meta-analysis of the architecture of AI-based systems and of the contexts in which AI-based components are to be reused to provide insights into what is safe to do.
          \draft{Which sub-discipline(s) does this come from?}
          
          Some stuff from Betty on views for personal information systems. ... A heterogeneous model combining several sources of information is also uninterestingly complex for a user to understand. Allowing exploration of complex knowledge of this kind requires an ability to perceive different fragments, known as views, of the model. The views need to be purpose specific, adaptive, and possibly synthesized on the fly, as the uses of the MEE model keep changing.
          \draft{Which sub-discipline(s) does this come from?}
          
          \draft{PIS} Probabilistic programs (models) allow integrating data and explicit knowledge but in an extremely limited form, and they require expert knowledge (statistics and probability).
          \draft{Which sub-discipline(s) does this come from?}
          
          The unification power of modeling through semantically rich abstractions and model interfaces offers great opportunities to support the identification and definition of arbitrarily complex alignments in between different domains. However, current technologies are tied to graph-structured abstractions and limit the application to other types of abstractions. The programming language (PL) community has a long history of integrating different kinds of abstractions (from classical dataflow analysis to abstract interpretation~\cite{cousot77} to a plethora of over-approximating~\cite{tonetta-svv06} and under-approximating~\cite{ascari-2022} abstractions and their combinations~\cite{albaghourthi-tacas12})  but they do not necessarily come with easily accessible notations. Another challenge is related to the integration, the interoperability and the complementarity of the different kinds of models embedded into a digital twin \cite{DBLP:journals/patterns/Blair21}. Model integration and interoperability face the challenge of taking care the uncertainty associated to the data collected from the actual system. The complementarity is specifically new in the context of digital twins, combining deductive and inductive reasoning through both analytical models and data models, all providing pros and cons (e.g., analytical models are usually explainable while data models are easily supported with data mining techniques). The consistency between them would help to detect some divergences in the running system with regards to the system as planned, and the collected data would also help in refining the initial analytical models. 
          \draft{Which sub-discipline(s) does this come from?}

    
    \item \emph{Reuse.}
    
          \draft{PIS} (Software Product Lines do not bite the bullet here, because they tend to have limited fixed variability; we need to generalize software product lines to self-evolve, not just deal with known unknowns.){\bf MC:  we should mention product lines as ways of handling known unknowns and managed evolution and say why this is great but not sufficient.  btw, nothing stops evolution of product lines from adding features, dynamic reconfiguration and adaptation, etc.}
          
          The closer are the domains of two digital twins, the more their core elements could be reused. Ideally, we should be able to define such core modeling abstractions for the DTs domain \cite{DTConcepts} and then use them to build Digital Twins as a composition, extension and customization of other existing Digital Twin components. This would also simplify their evolution as DTs are typically made for long-live systems, and, consequently, requirements on the system will change over time, forcing the DT to adapt to be able to respond to the new requirements \cite{AdaptiveChallenge}, including changes on the data they used, and how such data is modeled and explored by the end-users. If DTs are based on common abstractions, the evolution of the DT models and interfaces would automatically evolve as well all the DTs based on them.
          \draft{Which sub-discipline(s) does this come from?}

          \begin{itemize}
              \item
              As we have discucssed in the previous challenge, we are experts on capturing and formalizing semantically rich abstractions. But we are also able to manipulate such abstractions, for instance, comparing the abstractions in two related domains to find the common ground that could lead to opportunities for reuse and joint evolution. Indeed, we can envision the creation of a DT megamodel \footnote{A megamodel is a model of which at least some elements represent and/or refer to models or metamodels, including model transformations that could also be expressed as models \cite{bezivin2004need}} to conceptualize all aspects of set of DTs, their interrelationships and the interfaces to facilitate their interoperation. This could be basis for a number of key tasks such as the derivation of individual Digital Twins (following a kind of product-line approach for Digital Twins \cite{PLforDT}), or their automatic implementation thanks to the use of code-generation techniques. But this would also enable a more holistic/global reasoning by merging the data and simulations of individual DTs, required in larger initiatives like the DTs for cities or even for complete nations which should always be the result of a composition of local and sector-oriented DTs.

           %This includes standard interfaces for integrating with standard analyses, learned abstractions (from ML).
           %   \item Once such a model exists, we can apply ideas from model evolution to support the evolution over time.
           %   \item automating part of the DT dev. from design models
           %   \item DT composition for holistic / global reasonning
          \end{itemize}
          \draft{Which sub-discipline(s) does this come from?}

    
    \item \emph{Uncertainty.}
    
          While \emph{uncertainty} cannot be removed from AI-based systems, we can at least capture knowledge about the uncertainty in those systems that we are aware of.
          This can be done, among other things, by building \emph{arguments} of fitness for purpose rather than proofs of correctness.
          These structured arguments (similar to how safety assurance cases are built) can explicitly include models of uncertainty.
          \draft{Which sub-discipline(s) does this come from?}

  \end{enumerate}



  \draft{Needs integrating}

  \draft{Problem domain 1}
  
  \textbf{Known occurrences}

  \begin{draftlist}
    Betty, Marsha, can you provide some sentences and references here?
    
    \item Betty's work on goal modeling with GSN.  
    \item Marsha's work on reliability assurance cases for perception components.
    \item Tool:  MMINT-A:  combining behavioral and assurance models.
    \item Radu Calinescu:  assurance of ML lifecycle (AMLAS).          
  \end{draftlist}














  \section {[present successes] Core ideas/contributions of modeling research community}

    \begin {draftbar}
      Make it clear that modelling is not about boxes and arrows.

      Message: abstraction engineering (everybody agrees abstraction is key to computing, we enable abstraction in practice) (also modeling is very overloaded, which is another reason to prefer the term abstraction)

      Revisiting Is abstraction the key to computing?  \url{https://dl.acm.org/doi/abs/10.1145/1232743.1232745}

      Core ideas of modelling community: Abstraction, separation of concerns, systematic domain analysis, seeing systems through different views, understanding consistency, systematic understanding of abstractions (so designing languages is easy). We have patterns for common elements in languages (for instance modularization and reuse), and good principles for maintaining models (for instance traceability, no copy-paste modelling, etc.) We can contribute to the sustainability of software in many domains. We are experts in automation (code/doc/test generation, analysis, etc.).

Model management, especially of heterogeneous models:  composing, analyzing, querying related combinations of models of different types.

Co-evolution.  Code generation from models.

      All these practices and concepts allow to manage complexity
    \end {draftbar}

  \section {[future opportunities] Example areas where modeling can contribute}

    \begin {draftlist}
      TEMPLATE [ca. 1 page / 500 words]

      \item What is the exciting and challenging area/domain/problem you are trying to address. Use references from the relevant areas as a starting point to motivate, not modelling papers.
      \item What is the solution that you propose? Creating problem-solution pairs, including an outline of abstraction-based strategy
      \item What existing tech that already helps and open challenges for abstraction research
      \item What are the consequences of adopting the strategy (design pattern style)
    \end {draftlist}

    \draft{Betty suggested that we might want to find one application example that we can use in each of the three scenarios.}

    \subsection {[Betty \& Marsha] Trusting learning based systems (in Robotics or Autonomous Driving)}

      %\begin {draftlist}
        %This requires combining machine learned abstractions with abstractions modeled in assurance cases.
        %Betty's work on goal modeling with GSN.  Marsha's work on reliability assurance cases for perception components.  Tool:  MMINT-A:  combining behavioral and assurance models.
        %Radu Calinescu:  assurance of ML lifecycle (AMLAS).
%
        %\item Uncertainty
        %\item Multiple abstractions
        %\item data
      %\end {draftlist}
      %\begin{description}
          %\item[{Problem:}] \draft{Betty suggests to call these "problems" consistently to differentiate from the term "challenge" used in "open challenges" below}
                %\begin{enumerate}
                    %\item Challenge 1: Complexity
                          %\begin{itemize}
                              %\item Autonomous vehicles use AI to make decisions to navigate, to avoid accidents. Thus AI is used as a safety function.
                                %\item How do we assure the safety of these systems? They're crashing, but are we able to understand the causes and prevent these crashes?
                                %\item System is not human readable, no systematic process for development or evolution. Therefore, lack of traceability, formal analysis, assurance assessment, etc.
                                %\item System is complex and, therefore, traditional analysis based on hierarchical breakdown etc are not applicable and even notions of ``correctness'' in an absolute term may not be applicable. All we can do is reduce uncertainty\draft{Cite Ben Herd paper}.
                                %\item This is a challenge for explainable AI
                          %\end{itemize}
                    %\item Challenge 2: Combination / composition
                          %\begin{itemize}
                              %\item AI models are often used together, for example, to moderate between different classifiers
                              %\item Composing multiple different AI approaches requires deep expertise in each method
                          %\end{itemize}
                    %\item Challenge 3: Reuse and systematic development
                          %\begin{itemize}
                              %%\item When new training data arrives, you have to start from scratch and train the whole model again.
                              %%\item Every model starts from a blank state but there should be a way of reusing prior knowledge and approaches.
                              %\item How do we capture information about the QA that was done if we want to reuse an AI/ML component in a new context?
                              %\item The challenge that we can address is systematic development (assurance case modeling, test methods, etc.)
                          %\end{itemize}
                    %\item Challenge 4: Uncertainty \draft{How does this manifest specifically in this context?} \draft{Cf Betty's work on uncertainty interaction}
                            %\begin{itemize}
                                %\item Systems are put into unstructured environment, which provide create sources of uncertainty
                                %\item \emph{model uncertainty}: will the next prediction of the model be reliable based on previous predictions
                                %\item \emph{measurement uncertainty}: are the sensor data correct?
                                %\item \emph{unknown information about the world}: are the lane markings I can see meant to be there?
                                %\item \emph{composition of models}: how does uncertainty compose
                                %\item \emph{uncertainty about the system configuration}: end-user customisation creates design uncertainty about what software systems will play together
                                %\item \emph{training data uncertainty} did our training data accurately reflect the space of problems the system will be exposed to?
                                %\item \emph{specification uncertainty} there is no clear specification of what a hazard is
                            %\end{itemize}
                %\end{enumerate}
          %\item[{Solution Strategies: }]
          %\begin{description}
              %\item[{Preliminary Strategies: }]
              %\begin{itemize}
              %\item Betty's work on goal modeling with GSN.  \item Marsha's work on reliability assurance cases for perception components.
              %\item Tool:  MMINT-A:  combining behavioral and assurance models.
                %\item Radu Calinescu:  assurance of ML lifecycle (AMLAS).
               %\item Central ideas are about capturing the key abstractions in the system environment to allow a model-based testing-inspired approach, but then use evolutionary computation and model generation to produce as large and diverse and realistic a set of test scenarios as possible
                %\item GSN-based work is about building a declarative case about different properties of the system
                %\item Nelly mentioned her work on proxy models as a means to capture explicitly the non-intentional abstractions that an AI models has learned. Similarly, shielding in reinforcement learning allows to capture a safety envelope for the control strategy.
              %\end{itemize}
              %\item[{Open Challenges: }] \draft{What research in AE do we need to do to really make the solution strategies work?}
          %\end{description}
          %\item[{Context:}] Machine Learning systems based on neural networks (CNN, DNN, RL, etc.)
          %\item[{Consequences:}]
%
          %\item[{Known Occurrences: }]
      %\end{description}

      Modern systems increasingly include learning-based components.
      For example, autonomous cars include significant components for automated recognition and decision making, all of which are based on machine learning techniques.
      Widespread use of these technologies requires us to be able to trust them to ``do the right thing''.
      However, the systems often work as black boxes that don't easily allow analysis and inspection.
      
      \subsubsection{Problems}
      
        %\begin{draftlist}
          %\item Challenge 1: Complexity
                %\begin{itemize}
                  %\item Autonomous vehicles use AI to make decisions to navigate, to avoid accidents. Thus AI is used as a safety function.
                  %\item How do we assure the safety of these systems? They're crashing, but are we able to understand the causes and prevent these crashes?
                  %\item System is not human readable, no systematic process for development or evolution. Therefore, lack of traceability, formal analysis, assurance assessment, etc.
                  %\item System is complex and, therefore, traditional analysis based on hierarchical breakdown etc are not applicable and even notions of ``correctness'' in an absolute term may not be applicable. All we can do is reduce uncertainty\draft{Cite Ben Herd paper}.
                  %\item This is a challenge for explainable AI
                %\end{itemize}
          %\item Challenge 2: Combination / composition
                %\begin{itemize}
                  %\item AI models are often used together, for example, to moderate between different classifiers
                  %\item Composing multiple different AI approaches requires deep expertise in each method
                %\end{itemize}
          %\item Challenge 3: Reuse and systematic development
                %\begin{itemize}
                  %\item How do we capture information about the QA that was done if we want to reuse an AI/ML component in a new context?
                  %\item The challenge that we can address is systematic development (assurance case modeling, test methods, etc.)
                %\end{itemize}
          %\item Challenge 4: Uncertainty \draft{How does this manifest specifically in this context?} \draft{Cf Betty's work on uncertainty interaction}
                %\begin{itemize}
                  %\item Systems are put into unstructured environment, which provide create sources of uncertainty
                  %\item \emph{model uncertainty}: will the next prediction of the model be reliable based on previous predictions
                  %\item \emph{measurement uncertainty}: are the sensor data correct?
                  %\item \emph{unknown information about the world}: are the lane markings I can see meant to be there?
                  %\item \emph{composition of models}: how does uncertainty compose
                  %\item \emph{uncertainty about the system configuration}: end-user customisation creates design uncertainty about what software systems will play together
                  %\item \emph{training data uncertainty} did our training data accurately reflect the space of problems the system will be exposed to?
                  %\item \emph{specification uncertainty} there is no clear specification of what a hazard is
                %\end{itemize}
        %\end{draftlist}
        
        We identify four central problems in making AI-based systems more trustworthy:\draft{Give them unique labels (e.g., C1-1 to C1-4)?} \draft{Ensure that each problem is underpinned by concrete examples.}
        
        \begin{enumerate}
          \item \emph{Complexity.}
                AI-based systems, such as autonomous vehicles, use AI to make decisions in the real world (e.g., to navigate or to avoid accidents).
                AI is, therefore, a safety-relevant function in these systems and we should apply safety assurance methods.
                If an AI-based system malfunctions (e.g., if an autonomous system crashes), how can we understand the causes and prevent future malfunctions?
                Much of the behaviour of an AI-based system is not accessible to analysis because the system `implementation' is not readable to humans.
                Small changes to design or training can have significant changes -- this is characteristic of complex systems.
                As a result, these systems are not directly amenable to traditional formal analysis methods, which are often based on hierarchical breakdown.
                Even the notion of ``correctness'' as an absolute (rather than contingent) term may not be applicable.
          
          \item \emph{Compositionality.}
                AI models are often used together in the same system.
                For example, we may want to use multiple classifiers and base decisions on a majority vote between them to mitigate shortcomings of different types of classifiers.
                Alternatively, we may require different AI components to complete different tasks.
                For example, we may require a recognition component to identify objects in the street and a planning component to derive adaptations to the current navigation plan.
                However, composing different types of AI models in this way is not straightforward and requires significant expertise in each method to ensure the results can be trusted.
                
                Not only can AI models not be composed, we also cannot compose any evidence that captures any  assurance properties about a given AI-based component.
                For example, let's say that an obstacle detection subsystem has been assessed to work robustly in rain.
                We cannot combine that assessment with an assessment that the AI component works well in dark lighting conditions to claim that a given AI-based system works well in dark, rainy conditions.
                %Maybe your Reuse problem stated below is addressing this point? Although, the Reuse problem seems to refer to the usability of the AI component in a new context. Whereas my issue here is composition of assurance properties.}

          \item \emph{Reuse.}
                Once an AI-based system has been developed and quality assured, it is currently impossible to directly reuse the AI components in new contexts.
                This is because it is unclear which quality assurance outcomes can be transferred to the new context and which assurance activities have to be repeated.

          \item \emph{Uncertainty.}\draft{Cf Betty's work on uncertainty interaction}
                AI-based systems need to manage significant uncertainties both at design and at run time.
                These include:
                \begin{itemize}
                  \item \emph{Specification uncertainty:} 
                        Often, even the specification of what constitutes a `valid' result is vague in the case of AI-based systems.
                        In fact, AI-based systems are often employed specifically to manage such uncertainty.
                        However, if even the specification of what constitutes a hazard is uncertain, how can we successfully argue for system safety?
                  \item \emph{Environment uncertainty:} 
                        Systems are put into environments that expose high levels of uncertainty.
                        At design time, it is impossible to accurately capture all possible scenarios that a system may encounter.
                        At runtime, a system needs to cope with measurement uncertainty from its sensors.
                        There is also epistemic uncertainty about the environment.
                        For example, autonomous cars need to decide whether lane markings they identify are meant to be obeyed or are incompletely erased older markings (e.g. from a previous construction site).
                  \item \emph{Model uncertainty:}
                        Because of the black-box nature of learning-based systems, there is uncertainty about the functioning of the system itself.
                        In any given scenario, is the system still being used within the validity envelope determined by its training data?
                        High configurability of modern systems creates additional uncertainty as it becomes impossible at design time to predict all possible configurations and, therefore, all possible feature interactions.
                        Examples are the ability of drivers or passengers to connect their mobile phone to a car using a range of communication channels.
                        This adds an unpredictable range of software components to the system temporarily.
                \end{itemize}
                The problem of uncertainty is exacerbated as we compose systems from multiple AI components, where we then need to reason about how uncertainty composes.                
        \end{enumerate}
      
      \subsubsection{Abstraction Engineering solution strategies}
      
        %\begin{draftlist}
          %\item Central ideas are about capturing the key abstractions in the system environment to allow a model-based testing-inspired approach, but then use evolutionary computation and model generation to produce as large and diverse and realistic a set of test scenarios as possible
          %\item GSN-based work is about building a declarative case about different properties of the system
          %\item Nelly mentioned her work on proxy models as a means to capture explicitly the non-intentional abstractions that an AI models has learned. Similarly, shielding in reinforcement learning allows to capture a safety envelope for the control strategy.
        %\end{draftlist}
        
        Several strategies can be applied to address these problems:
        
        \begin{itemize}
          \item The \emph{complexity} of AI-based systems and their environments can be partially addressed by capturing key abstractions of the system environment (e.g., roads, pavements, pedestrians\ldots) so that a broad variety of large, diverse, and realistic test scenarios can be automatically generated using evolutionary computation and model generation. 
                While this may not be able to provide the level of assurance that model-based testing can provide for more traditionally engineered systems, the level of assurance can be increased by generating as broad and diverse a range of scenarios as possible.
          \item Issues of \emph{compositionality} and \emph{reuse} can be addressed by capturing key abstractions about how AI-based components are engineered and how they may interact with other components.
                This will enable meta-analysis of the architecture of AI-based systems and of the contexts in which AI-based components are to be reused to provide insights into what is safe to do.
          \item While \emph{uncertainty} cannot be removed from AI-based systems, we can at least capture knowledge about the uncertainty in those systems that we are aware of.
                This can be done, among other things, by building \emph{arguments} of fitness for purpose rather than proofs of correctness.
                These structured arguments (similar to how safety assurance cases are built) can explicitly include models of uncertainty.
        \end{itemize}
        
      
      \subsubsection{Challenges}
      
        \draft{What research in AE do we need to do to really make the solution strategies work?}
      
      \subsubsection{Known occurrences}

        \begin{draftlist}
          Betty, Marsha, can you provide some sentences and references here?
          
          \item Betty's work on goal modeling with GSN.  
          \item Marsha's work on reliability assurance cases for perception components.
          \item Tool:  MMINT-A:  combining behavioral and assurance models.
          \item Radu Calinescu:  assurance of ML lifecycle (AMLAS).          
        \end{draftlist}
      

\subsection {[Marsha \& Andrzej \& Nelly] Combining Explicit and Implicit Knowledge }


\noindent
% Not only factories, robots, and smart cities can benefit from modeling and analysis of what-if scenarios.  
Ergonomic access to generalized and personalized information can empower any modern human in personal and professional decision making.  Envision a personalized adaptive information service\,\cite {DBLP:conf/models/MussbacherABBCCCFHHKSSSW14} for individuals and small groups, offering a simple analytical tool for decision making regarding travel planning, tax returns, day-to-day economy, smart house control, etc.  For instance, the system can learn from your behaviors that you tend to cook for a larger group of people in the weekends, and suggest a recipe and shopping list knowing the content of your fridge, and how many of the coming friends are vegetarian. Or a car may learn the acceleration, breaking, and safety distance profile you like, combining it with the knowledge of the driving code at a location where you are.

Solving such problems requires combing \emph{explicit symbolic knowledge} (your calendar, scanning of objects in the fridge, model of dietary preferences) with the \emph{implicit statistical knowledge} (adaptive, learned models of your driving preferences, shopping preferences, and cooking habits).

\subsubsection {Problems}

      
      \begin{itemize}

        \item \emph{Complexity}. A personalized information service needs to deal with complexity of essentially unbounded knowledge in your life. In order to maintain the ergonomy of interaction it needs to arrive at \emph{personalized abstractions} that present only the required information, in a manner that is comprehensible for the individual user. Furthermore, when the user is interested in more detailed information as provided, automatic refinement of the presented abstractions is needed. Note that the activities of abstraction and refinement of information are key activities in Abstraction Engineering. 

        \item \emph{Compositionality}. Models in personal information system are partial and dynamic, not necessary prescriptive. Some are human made-some are machine-learned. The issue of compositionality lies at the heart of information management, where explicit models, databases, and machine learning models are to be composed into a single functioning system. Presently, the generative models, large data sets, and explicit information models live in separate silos, and indeed researchers are challenged on how to combine them effectively, and how to allow explicit knowledge to override implicit knowledge (for instance for what-if analysis). Moreover there is a tension between  the algorithmic query answering mechanisms  vs a conversational interfaces of Large Language Models. Knowledge is not easily composable, not only because of different contexts. Tensions exists between different priorities: for instance is your diet more important or is the general climate data more important? 
       
        \item \emph{Reuse.} We presently do not have modeling and knowledge architectures that allow to arrive at such a personalized adaptive information system in a single uniform implementation. The fields of modeling, information management, programming languages need to work out the solutions how to build systems that abstract from an individual user in the implementation, but are highly adaptive and idiosyncratic at runtime. 

        \item \emph{Uncertainty.} ... , abstraction levels, representations, but also because of different levels of trustworthiness and certainty ...


      \end{itemize}
      
      \subsubsection{Abstraction Engineering Solution Strategies}

      \begin {itemize}

        \item known unknowns, unknown unknowns (different abstractions methods needed)

        \item  No idea?

        \item Some stuff from Betty on views. ... A heterogeneous model combining several sources of information is also uninterestingly complex for a user to understand. Allowing exploration of complex knowledge of this kind requires an ability to perceive different fragments, known as views, of the model. The views need to be purpose specific, adaptive, and possibly synthesized on the fly, as the uses of the MEE model keep changing.

        \item Probabilistic programs (models) allow integrating data and explicit knowledge but in an extremely limited form, and they require expert knowledge (statistics and probability).

        \item Reuse: (Software Product Lines do not bite the bullet here, because they tend to have limited fixed variability; we need to generalize software product lines to self-evolve, not just deal with known unknowns. TODO: perhaps move this remark to solutions)

      \end {itemize}


    \subsection {[Jordi \& Steffen \& Nelly \& Benoit] Digital Twins}

      \begin {draftlist}
        \item (on the example of Nation-wide DT in Lux, smart infrastructure; what if scenarios, measurements), making DT development a discipline, so that the tech is reusable, so that DT and data can (co-)-evolve, so that the DTs can be integrated (federated)
        \item Nation-wide digital twins as composition of sector-specific twins
        \item DTs can provide support for reasoning at given levels of abstraction
      \end {draftlist}

      \begin{itemize}
          \item A modern smart city needs digital instruments to plan mobility, traffic management, control pollution, crowd management, ... . Digital Twins is a technology that may help cities to adapt to the fast changing reality \footnote{\url{https://www3.weforum.org/docs/WEF_Global_Digital_Twin_Cities_Framework_and_Practice_2022.pdf}}.
          \item Complex embedded systems (e.g. aircraft) are involving in a continuously evolving and changing environment, and need to adapt. It also need to be optimized in such an environment, wrt. performances, energy consumption, etc.
          \item A key aspect of DTs is that they enable analysis (including what--if/if--what analysis, trade-off analysis, design space exploration, decision making). Different stakeholders will be interested in analysis at different levels of granularity (e.g., whole-city view vs transport-system view) and levels of abstraction.
      \end{itemize}

      \subsubsection{What is the exciting and challenging area/domain/problem you are trying to address.} \draft{Use references from the relevant areas as starting point to motivate, not modelling papers.}

      Representative challenges where modelling is going to be useful:

      \begin{itemize}
          \item Challenges:\draft{Possibly swap Challenges 1 and 2}
                \begin{enumerate}
                    \item \label{DT-Challenge-1} {NELLY TO DO} Complexity of DTs as software systems -- how to balance the need of users to understand enough about what the DT does and represents without needing to become software experts, including how do the human users trust the DT
                    \item  \label{DT-Challenge-2} Digital Twins embed different models to support the various services to be provided to the end-users. These models can play different roles, possibly over the time, to support the different expected services \cite{eramo:hal-03466396}. In particular, the representation of the system requires descriptive models, to be used in combination with predictive models for conducting predictive simulation, and possibly with prescriptive models to act back on the system. While some models can be borrowed from design time, some others required to be defined and built at runtime. Another challenge consists in the data to be collected by the digital twin from the raw data provided by the physical system. This must be done possibly with a specific frequency, some uncertainty, and complex event processing to deliver the right level of abstraction to the digital twin. 
                    \item  \label{DT-Challenge-3} We have seen an explosion of digital twins (for mobility, for electricity consumption, for industrial plants, for water monitoring, etc). But each of them is modeled and built from scratch, even if, clearly, all digital twins share a set of common blocks. The closer are the domains of two digital twins, the more their core elements could be reused. Ideally, we should be able to define such core modeling abstractions for the DTs domain \cite{DTConcepts} and then use them to build Digital Twins as a composition, extension and customization of other existing Digital Twin components. This would also simplify their evolution as DTs are typically made for long-live systems, and, consequently, requirements on the system will change over time, forcing the DT to adapt to be able to respond to the new requirements \cite{AdaptiveChallenge}, including changes on the data they used, and how such data is modeled and explored by the end-users. If DTs are based on common abstractions, the evolution of the DT models and interfaces would automatically evolve as well all the DTs based on them.

                      %OLD TEXT FOR REF:      %Reusable technology for developing digital twins -- currently everything is bespoke -- needs to support evolution, reusability, and customisation
                    %Evolution is particularly relevant here as DTs are typically made for long-lived systems  and thus, the models and data needed to answer these questions. We don't have all the answers for this, but there are works that have considered model evolution etc and identified the challenges that have to be considered and some solutions.
                    %Includes also building DTs from composition of other DTs.
                    % Bespoke systems are hard to interface to general exploration and optimization methods (due to lack of interfaces and abstractions).

                \end{enumerate}
      \end{itemize}

      \subsubsection{What is the solution you are proposing? Creating problem-solution pairs, including an outline of abstraction-based strategy}

        \begin{enumerate}
            \item For Challenge~\ref{DT-Challenge-1}:
                  \begin{itemize}
                      \item Some of this is `bread and butter': we know how to build modelling languages/notations and domain-relevant abstractions that can hide complexity as well as transformations for translating these into executable software. It is worth mentioning that we can provide different notations for different profiles, all linked to the same metamodel.
                      \item We also have existing and emerging technology to support collaboration between stakeholders with different views (though  reconciliation where conflict occurs and possibly across abstraction levels needs more support)\draft{Add some references here} as well as their efficient near-realtime collaboration\draft{possibly cite web-based modelling}
                      \item It remains to better support the human in the loop by finding better ways of identifying the \emph{right} abstractions.
                      \item Having the right abstractions and models to communicate information pertaining to trustworthiness of the DT remains an open challenge -- we know how to build abstractions, and GSN-style languages may be particularly promising here -- but we don't know the specific abstractions we need. We need ways to expose complexity/causality in a DT in limited but useful ways to explain and document decision making.
                  \end{itemize}
            \item For Challenge~\ref{DT-Challenge-2}:
                  The unification power of modeling through semantically rich abstractions and model interfaces offers great opportunities to support the identification and definition of arbitrarily complex alignments in between different domains. However, current technologies are tied to graph-structured abstractions and limit the application to other types of abstractions. The programming language (PL) community has a long history of integrating different kinds of abstractions\draft{Marsha can provide pointers?} but they do not necessarily come with easily accessible notations. Another challenge is related to the integration, the interoperability and the complementarity of the different kinds of models embedded into a digital twin \cite{DBLP:journals/patterns/Blair21}. Model integration and interoperability face the challenge of taking care the uncertainty associated to the data collected from the actual system. The complementarity is specifically new in the context of digital twins, combining deductive and inductive reasoning through both analytical models and data models, all providing pros and cons (e.g., analytical models are usually explainable while data models are easily supported with data mining techniques). The consistency between them would help to detect some divergences in the running system with regards to the system as planned, and the collected data would also help in refining the initial analytical models. 
            \item For Challenge~\ref{DT-Challenge-3}:
                  \begin{itemize}
                      \item
                      As we have discucssed in the previous challenge, we are experts on capturing and formalizing semantically rich abstractions. But we are also able to manipulate such abstractions, for instance, comparing the abstractions in two related domains to find the common ground that could lead to opportunities for reuse and joint evolution. Indeed, we can envision the creation of a DT megamodel \footnote{A megamodel is a model of which at least some elements represent and/or refer to models or metamodels, including model transformations that could also be expressed as models \cite{bezivin2004need}} to conceptualize all aspects of set of DTs, their interrelationships and the interfaces to facilitate their interoperation. This could be basis for a number of key tasks such as the derivation of individual Digital Twins (following a kind of product-line approach for Digital Twins \cite{PLforDT}), or their automatic implementation thanks to the use of code-generation techniques. But this would also enable a more holistic/global reasoning by merging the data and simulations of individual DTs, required in larger initiatives like the DTs for cities or even for complete nations which should always be the result of a composition of local and sector-oriented DTs.

                   %This includes standard interfaces for integrating with standard analyses, learned abstractions (from ML).
                   %   \item Once such a model exists, we can apply ideas from model evolution to support the evolution over time.
                   %   \item automating part of the DT dev. from design models
                   %   \item DT composition for holistic / global reasonning
                  \end{itemize}
        \end{enumerate}

        % TO BE ASKED TO STEFFEN:
      %\subsubsection{What existing tech that already helps and open challenges for abstraction research}

        %\draft{Should this section be combined with the above?}

      %\subsubsection{What are the consequences of adopting the strategy?}



  \section {Conclusions}

    \draft {[closing message] Help us help you—we want to grow—research challenges; Need a pitch for why people should join us.}



==> problem_domains-backup.tex <==
\section {Abstraction in Contemporary Computing}%
\label {section:problem_domains}

Let us consider three examples of modern computing systems. Each of these captures a different point in the abstraction-engineering design space.  We ask the same six questions for each of them, based on the ``5 w's and h'' framework. % (who, what, when, where, why, how):
\draft{AW: somehow this became the 6 w's and h's framework, not five ...}

\begin{enumerate}

    \item \emph{How?} Is the abstraction \emph{designed} in a top-down fashion or is it \emph{discovered}?
          % SZ: Removed the next bit; I think it's covered by "why" already.
          %Because of a particular analysis need or via an interaction with humans or other components?

    \item \emph{Who?} Who creates the abstraction, a \emph{human} or a \emph{machine}?

    \item \emph{When?} Is the abstraction \emph{static} throughout the life of the software system, or is it \emph{adaptive}; that is, does it change as the software evolves?
          %In other words, when? will the abstraction change?

    \item \emph{Where?} At what stage of the software lifecycle is the abstraction defined and used: \emph{design time} or \emph{run time}?
       \draft{NB: it can also be seen as when? perhaps needs to be expressed differently}\draft{SZ: I agree, this is the one I'm least happy with.}
       \draft{AW: Also think this is fishy. Should we perhaps just merge with when, and drop the explicit dependency on the 5 w\&h framework?}

    \item \emph{Why?} Why was the abstraction created (e.g., to manage complexity, to enable analysis, serve as a communication vehicle between stakeholders, support development/maintenance, etc.)?.
      \draft{AW: I somehow feel that Why is asked waay too late. I would consider asking it first? Similarly with What? These seem to be the basic questions}\draft{SZ: I agree, reordering makes sense}

    \item \emph{What?} What is being abstracted?

\end{enumerate}
\draft{Arguably, these dimensions are themselves already a first contribution of AE.}
%
Some abstractions have multiple answers to a question. For example, an abstraction may be created by a human but refined by a machine.

\subsubsection* {Trusting learning based systems (Robotics and Autonomous Driving)}

  % \draft{Betty, Marsha, Steffen}
  Machine-learning-based components are responsible for automated recognition and decision making in autonomous cars.  In fact not just cars, but many modern systems include \emph{learning-enabled components} (LECs). Widespread use of these technologies requires us to be able to trust them to ``do the right thing''. However, the systems often work as black boxes that are not amenable to traditional analysis and inspection techniques. An inherent property of LECs is the reliance on training data, which can pose significant challenges when the operating environment was not captured in the training data.


  Abstractions can be used in two complementary ways when addressing assurance of AI-based systems. First, due to the lack of human-readable form of AI components, abstract representations are needed to capture the intended behavior of the LECs (both functional and non-functional objectives), which need to be amenable to automated analysis. Second, abstractions are needed to capture assurance objectives, strategies for achieving these objectives, and evidence that these objectives have been satisfied.  With these two perspectives in mind, we illustrate the respective abstract dimensions.
  \paragraph {Behavior/Requirements Specification of Learning-enabled Components}
  \draft{SZ: What's special to AI about these statements? This text feels like it could be written pretty much the same way for the requirements and design of pretty much any system.}
  \begin{itemize}
   \item {\it How:} Abstractions are needed to capture observable behavior, which will likely require domain experts to apply a top-down approach to create the appropriate models.
   \item {\it Who: } Abstractions are created by requirements engineer and/or domain experts.
   \item {\it When: } Requirements are specified in a static fashion to capture dynamic information. The requirements-based abstractions typically do not change at run time. The challenge is how to engineer the abstractions to ``accurately'' represent the behavior of the system as it executes and responds to the changing environmental conditions.
   \item {\it Where: } Heavier-weighted analysis techniques can be used at design time to analyze system requirements abstractions for adherence to assurance\draft{SZ: I thought assurance is the next example?} properties. In contrast, lighter-weight techniques are needed to analyze limited portions of the abstraction models for assurance at run time.
   \item {\it What: }Abstractions are capturing functional and non-functional requirements of system

  \end{itemize}

\paragraph {Assurance Requirements for LECs}
\draft{SZ: It would be good if this could show what's AI-specific rather than `just' regular safety assurance.}
\begin{itemize}
     \item {\it How:} Abstractions need to specify assurance properties, strategies, and evidence needed to establish/satisfy assurance properties.\draft{SZ: The `how' question is about top-down vs bottom-up. Which of these is relevant here?}
     \item {\it Who: } Abstractions are created by requirements engineers, domain experts, and quality assurance engineers.
     \item {\it When: } Assurance case models are traditionally not intended to change at runtime,  but work is emerging to update evidence used to establish assurance.
     \item {\it Where: } Most analysis assurance abstractions are performed at design time. Emerging techniques are exploring the run-time analysis of assurance case models at run time.  {\bf MC:  this is same as above}
     \item {\it What: } Abstractions are capturing assurance case properties, assurance strategies, and assurance evidence.
    \end{itemize}

\subsection* {Combining Explicit and Implicit Knowledge} \draft{in Title of section: are these the terms we want to use? they are not used in the paragraph}
  \label{section:problem_domains:pais}

    \draft{Marsha, Andrzej, Nelly, Betty}

    Ergonomic \draft{Ergonomic? is this the term we want to use?}  {\bf MC:  I do not like the term.  "Effective"?  "Integrated"?} access to generalized and personalized information can empower any modern human in personal and professional decision making.
    Envision a personalized adaptive information service~\cite{DBLP:conf/models/MussbacherABBCCCFHHKSSSW14} for individuals and small groups, offering a simple analytical tool for decision-making regarding travel planning, tax returns, day-to-day economy, smart house control, etc.
    For instance, the system can learn from the user behaviors that she tends to cook for a larger group of people in the weekends, and suggest a recipe and shopping list knowing the content of her fridge, and how many of the coming friends are vegetarian.
    Or a car may learn the acceleration, breaking, and safety distance profile its driver likes, combining it with the knowledge of the driving code at a location where she is.

    Solving such problems requires combining \emph{explicit symbolic knowledge} (your calendar, scanning of objects in the fridge, model of dietary preferences) with \emph{implicit statistical knowledge} (adaptive, learned models of your driving preferences, shopping preferences, and cooking habits).
    {\bf MC:  do we do the 5W and H analysis here?}\draft{\textbf{YES, MARSHA PLEASE ADD THIS HERE!!!!}}

  \paragraph {Digital Twins}

    \draft{Jordi, Steffen, Nelly, Benoit}

A \emph{digital twin} (DT) is a digital representation of a complex physical object, system or process. For instance, a city-wide DT would cover the modeling of mobility, electricity, pollution,... patterns across the city. A key aspect of DTs is that they enable simulation and analysis (including what--if/if--what analysis, trade-off analysis, design space exploration, decision making) of the real elements.  Different stakeholders will be interested in analysis at different levels of granularity (e.g., whole-city view vs transport-system view) and levels of abstraction.

Given the different roles and scenarios where a DT could be useful, DTs are a great example to illustrate the previous abstraction dimensions:
\begin{itemize}
\item \textit{How}: abstractions in a DT are both created and discovered. Indeed, some abstractions are created with the help of domain experts that decide what elements of the real-world objects are important for the DT purpose and therefore need to be part of the abstractions. Others are discovered when connecting to the DT sources of data (mainly sensors and other real-time data inputs) whose schema and patterns are dynamic and need to be discovered
\item \textit{Who}: Mostly humans though the discovery part could be partially automated and then human-reviewed before merging it into the manually created abstractions
\item \textit{When}: Again, both. Digital twins can be very long-lived, alongside the real system they are `twinning'. We start with an initial abstraction that must evolve over time as the real system also evolves.
\item \textit{Where}: Most DTs will be used through the whole life cycle of the modeled system as a tool to constantly analyze and simulate changes on the DT of the system that could be then put in the place on the real system to improve it.
\item \textit{What}: This will largely depend on the DT but, typically, we will be abstracting both the data managed/consumed by the system (``models \emph{in} a digital twin'') and the processes reading and updating such data (``models \emph{of} a digital twin'').

\end{itemize}

    %\begin {draftlist}
      %\item (on the example of Nation-wide DT in Lux, smart infrastructure; what if scenarios, measurements), making DT development a discipline, so that the tech is reusable, so that DT and data can (co-)-evolve, so that the DTs can be integrated (federated)
      %\item Nation-wide digital twins as composition of sector-specific twins
      %\item DTs can provide support for reasoning at given levels of abstraction
    %\end {draftlist}
%
    %\begin{itemize}
      %\item A modern smart city needs digital instruments to plan mobility, traffic management, control pollution, crowd management, ... . Digital Twins is a technology that may help cities to adapt to the fast changing reality \footnote{\url{https://www3.weforum.org/docs/WEF_Global_Digital_Twin_Cities_Framework_and_Practice_2022.pdf}}.
      %\item Complex embedded systems (e.g. aircraft) are involving in a continuously evolving and changing environment, and need to adapt. It also need to be optimized in such an environment, wrt. performances, energy consumption, etc.
      %\item A key aspect of DTs is that they enable analysis (including what--if/if--what analysis, trade-off analysis, design space exploration, decision making). Different stakeholders will be interested in analysis at different levels of granularity (e.g., whole-city view vs transport-system view) and levels of abstraction.
    %\end{itemize}


==> solution_strategies.tex <==
\section {Solution Strategies}%
\label {section:solution_strategies}

  %% SZ: Old text moved to start of _text_mine.tex

% should be a positive text to integrate work done in other areas to our crusade

% a breath of applications have been identified

% Jordi's examples
\textbf{Jordi}: To help with the uncertainty challenge, we propose to adapt probabilistic extensions to binary logic that can help experts express the degree of belief in the elements in an abstraction. In particular, we believe that
Subjective logic, by Audun Jøsang~\cite{Josang01}, would be particularly useful as this is a type of probabilistic logic that explicitly takes uncertainty into account. Even more, subjective opinions can be used to express beliefs and disbeliefs about the truth of propositions under degrees of uncertainty. So, it allows users to express both the uncertainty of the elements (e.g., because they come from inference on data samples) and their confidence on the uncertainty values  of those elements.  {\bf MC:  this one seems to crosscut - enable widespread usage of probabilistic logic that captures the uncertainty, confidence, etc.  This is a multifaceted challenge:  need specification languages, reasoning, testing, monitoring - the whole nine yards with such logics}

\textbf{Jordi}: I think product lines~\cite{van2007software} could be another example solution technique for the compositionality / reuse challenge as it would help us to reuse abstractions and compose them for new projects.  {\bf MC : Product lines are specifically developed to facilitate reuse. "Managed evolution". The interesting abstraction here is feature as a unit of functionality or a unit of variability.  The community learned a lot about how to do it well. Some of the work - movement of features across project branches, eg, in git - explicitly supports our goals}

\textbf{Jordi}: Theoretical computer science concepts could help in classifying how complex is an abstraction (related to the complexity challenge)  so that we also understand what manipulations can be done with it.  {\bf MC:  this might be too vague. do you mean that we can study best, worst and expected running times of well understood abstractions, as we have done with red-black trees or map-reduce, and organize them in some libraries for reuse? Or do we mean validated solution templates that can be configured for a particular purpose and we get correctness / performance guarantees?}


\paragraph {Andrzej}: The complexity of decision-making by modern AI based system can be tackled using probabilistic modeling. For testing purposes \cite{???}, and diagnosis purposes \cite{???} the deterministic neural systems can be described as much simpler probabilistic system.  In some way, this trades complexity for uncertainty, but if the uncertainty is low enough to test and verify relevant properties, this abstraction can be used effectively \cite{}.   {\bf MC: same point as Jordi's}
% I do not have these citations, but I am sure I can find them if start googling.

\paragraph {Andrzej}: The uncertainty problem is already being tackled by early works in the testing~\cite{MAYBEICFP23}, verification~\cite{MAYBECEASAR}, and requirements engineering~\cite{SOTIF} for systems displaying probabilistic behaviors or operating in uncertain conditions. However, these methods are still at the early stages.  We do not know which properties over which abstractions (models) are testable; the verification procedures are far from being able to handle complex probabilistic abstractions, and the requirements engineering methods still typically follow the enumerative approach used in the past for deterministic systems,  i.e., enumerating scenarios and behaviors, a process which is very hard to scale to the complexity of modern autonomous systems.

%\textbf{Example proposed by Nelly}
% \textbf{Problem}: the need to support the dynamic generation of software artefacts at execution time. For example, the generation of software mediators to tackle the crucial interoperability problem in modern software-based systems (known asemergent interoperability software). Therefore, there is a need to construct, at runtime, emergent abstractions that can support the interoperability need that couldn’t be foreseen before.

\textbf{Nelly}: AI-based modern software requires a fundamentally new approach to resolving compositionability (BHC: composability? compositionality?) and associated interoperability problems during executions (runtime).  Runtime models can be used to deal with these issues:  during execution runtime models can be defined as abstract representations of the needed system components, including their structure and behaviour.
A challenge is to come up with the abstractions that would require support communications between the two or more systems.  We foresee that ontological information to enable semantic reasoning would be required~\cite{Bencomo2013}.
%and UQ and reasoning for decision-making

\textbf{Benoit}:
Abstraction engineering is the heart and soul of \emph{Software Language Engineering} \cite{10.5555/1496375}, whose the main objective is to engineer tool-supported abstractions in so-called domain-specific (modeling) languages~\cite{mdebook,dsldesign}. Abstractions are thus promoted at the level of language constructs to be supported by tools and used to define any specific instances.
%
In this context, numerous works have been done in the past decades on language reuse
~\cite{butting2020compositional} as a way of reusing abstractions from one domain to another. Similarly, language composition operators~\cite{10.1145/2427048.2427055}  are used to align and complement abstractions from different domains.

\textbf{Marsha}: Abstraction has been a key concept in the verification community   from defining automated reasoning over useful "fixed" abstraction via \emph{abstract interpretation} to dynamically discovering abstractions through counter-example-based abstraction refinement (CEGAR) approaches to software verification.  The goal was less about managing uncertainty or enabling reuse but defining abstractions that are small enough to enable decision procedures and yet precise enough so that analysis results can be meaningful.  Scalable solutions for reasoning over probabilistic and possibilistic systems, capturing uncertainty, have also been developed by this community~\cite{prism,albarghouthi12,dippolito08}.



\textbf{XXXX}: Software Architecture: TODOs

 \begin{draftlist}
      Please add a paragraph per example following the structure below. You can add multiple examples, one paragraph each.

      \item Provide a short description of the example (a couple of sentences should be enough)
      \item Provide a reference to a paper/papers with the details
      \item State which challenge(s) in which problem domain(s) are addressed in which way
  \end{draftlist}

  \paragraph {SZ: An example on digital twins}
  Digital twins are complex software systems that represent complex real-world systems.
  To manage the complexity, make the development of digital twins manageable, and the final twins understandable to domain experts, it is important that the right abstractions are used in the description of the digital twins themselves, and importantly the real-world system they represent.
  In different areas, this strategy has been applied already.
  For example, the Asset Administration Shell (AAS)~\cite{AAS} developed by the Industrial Digital Twin Association is a set of meta-models and sub-model specifications covering a wide range of data schemas for digital twins in the manufacturing industry.
  In the context of socio-technical digital twins, \cite{Godfrey+23} is an example of a domain-specific modelling language for modelling and simulating emergency-care work processes.
  Such DSML-based approaches not only address the challenge of managing \emph{complexity}, they also enable the \emph{reuse} of knowledge from one digital twin to the next or as requirements for an existing digital twin change over time.

